Low-rank Interaction with Sparse Additive Effects Model for Large Data Frames

Many applications of machine learning involve the analysis of large data frames-matrices collecting heterogeneous measurements (binary, numerical, counts, etc.) across samples-with missing values. Low-rank models, as studied by Udell et al. [30], are popular in this framework for tasks such as visualization, clustering and missing value imputation. Yet, available methods with statistical guarantees and efficient optimization do not allow explicit modeling of main additive effects such as row and column, or covariate effects. In this paper, we introduce a low-rank interaction and sparse additive effects (LORIS) model which combines matrix regression on a dictionary and low-rank design, to estimate main effects and interactions simultaneously. We provide statistical guarantees in the form of upper bounds on the estimation error of both components. Then, we introduce a mixed coordinate gradient descent (MCGD) method which provably converges sub-linearly to an optimal solution and is computationally efficient for large scale data sets. We show on simulated and survey data that the method has a clear advantage over current practices, which consist in dealing separately with additive effects in a preprocessing step.

==> theory.tex <==
\section{Statistical results}
\label{theory}

In this section we give upper bounds on the estimation error of estimator \eqref{optim}. These results are deepened and extended in \cite{robin} where the reader can find the proofs as well as corresponding lower bounds. 

\paragraph{Assumptions and notations}
We now describe our main assumptions on the parameters $\alp^0$ and $\mathbf{\Theta^0}$, the distribution of the noise and sampling, and on the dictionary. Define $\mathcal{I} = \{k\in [n]; \alp_k\neq 0\}$, and let $a>0$.
\begin{assumption}\label{ass:ident}
$\norm{\alp}_{\infty}\leq a$ and $\norm{\mathbf{\Theta}^0}_{\infty}\leq a$.
Furthermore, for all $k\in \mathcal{I}$, $\pscal{\mathbf{\Theta}^0}{\mathbf{X}(k)} = 0$.
\end{assumption}
Assumption \Cref{ass:ident} guarantees the identifiability of model \eqref{exp-model}; note that we do not assume that $\mathcal{I}$ is known. Denote by $\mathbf{G}_{\mathbf{X}}$ the Gram matrix with entries $\mathbf{G}_{\mathbf{X}}(k,l) = \pscal{\mathbf{X}(k)}{\mathbf{X}(l)}$. We make the following assumption on the dictionary.
\begin{assumption} \label{ass:dict}
For all $(i,j)\in[n]\times [p]$, $\sum_{k=1}^q |\mathbf{x}_{ij}(k)|\leq 1$. Furthermore, there exists $\kappa^2\geq 0$ for all $\alp\in\mathbb{R}^q$, 
$$\alp^{\top} \mathbf{G}_{\mathbf{X}}\alp >\kappa^2\norm{\alp}_2^2.$$
\end{assumption}
%Assumption \Cref{ass:dict} implies that if $\norm{\alp}_{\infty}\leq a$ and $\norm{\mathbf{\Theta}}_{\infty}\leq a$, then $\norm{\sum_{k=1}^q\alp_k\mathbf{X}(k) + \mathbf{\Theta}}_{\infty}\leq 2a$. In particular, this is satisfied if the covariate vectors $\mathbf{x}_{ij}$ are indicators of categorical variables.\\
 Let $(\mathbf{E}_{11}, \ldots , \mathbf{E}_{np})$ be the canonical basis of $\mathbb{R}^{n\times p}$. For $\mathbf{M}\in\mathbb{R}^{n\times p}$, we denote the negative log-likelihood of the observed data $(\mathbf{Y}, \Omega)$ parametrized by $\mathbf{M}$ and its gradient with respect to $\mathbf{M}$ as follows:
$$\mathcal{L}(\mathbf{M}) = \sum_{(i,j)\in \Omega}\left\lbrace-\mathbf{Y}_{ij}\mathbf{M}_{ij}+g_j(\mathbf{M}_{ij})\right\rbrace,\quad\nabla \mathcal{L}(\mathbf{M}) = \sum_{(i,j)\in \Omega}\left\lbrace-\mathbf{Y}_{ij}+g_j'(\mathbf{M}_{ij})\right\rbrace \mathbf{E}_{ij}.$$
\begin{assumption} \label{ass:strong-cvx}
For all $1\leq j\leq p$, $g_j$ is twice differentiable; furthermore there exist constants $\sigma_{+}$, $\sigma_{-}$ and $\gamma$ such that for all $x\in [- 2a - \gamma, 2a + \gamma]$, 
$$\sigma_{-}^2\leq g_j''(x)\leq  \sigma_{+}^2.$$
\end{assumption}
Denote $\norm{\mathbf{M}}_{\Omega}^2 = \sum_{(i,j)\in \Omega} \mathbf{M}_{ij}^2$.
Assumption \Cref{ass:strong-cvx} has two important consequences. First, the negative log-likelihood $\mathcal{L}$ satisfies some restricted convexity; for all $\mathbf{M}_1$ and $\mathbf{M}_2$ in $\mathbb{R}^{n\times p}$:
$$\mathcal{L}(\mathbf{M}_2) -  \mathcal{L}(\mathbf{M}_1) - \pscal{\nabla \mathcal{L}(\mathbf{M}_1)}{\mathbf{M}_2-\mathbf{M}_1}\geq \frac{\sigma_{-}^2}{2}\norm{\mathbf{M}_2-\mathbf{M}_1}_{\Omega}^2.$$
Second, the entries $\mathbf{Y}_{ij}$ are sub-exponential random-variables with scale and variance parameters $1/\gamma$ and $\sigma_{+}^2$ respectively; for all $(i,j)\in[n]\times[p]$ and for all $z\in\mathbb{R}$, $|z|<1/\gamma$, $\mathbb{E}\left[\mathrm{e}^{z(\mathbf{Y}_{ij}-\mathbb{E}[\mathbf{Y}_{ij}])}\right]\leq \mathrm{e}^{\frac{\sigma_+^2z^2}{2}}$.\\
\begin{assumption}{(Almost uniform sampling)} \label{ass:sampling} 
$\omega_{ij} = \{(i,j)\in\Omega\}$, $(i,j)\in [n]\times [p]$ are independent Bernoulli random variables, and there exist $\pi >0$ such that for all $(i,j)\in [n]\times [p]$, 
$$ \mathbb{P}(\omega_{ij}) > \pi.$$
\end{assumption}

